Directed Graph Minors and Serial-Parallel Width

Graph minors are a primary tool in understanding the structure of undirected graphs, with many conceptual and algorithmic implications. We propose new variants of \emph{directed graph minors} and \emph{directed graph embeddings}, by modifying familiar definitions. For the class of 2-terminal directed acyclic graphs (TDAGs) our two definitions coincide, and the class is closed under both operations. The usefulness of our directed minor operations is demonstrated by characterizing all TDAGs with serial-parallel width at most $k$; a class of networks known to guarantee bounded negative externality in nonatomic routing games. Our characterization implies that a TDAG has serial-parallel width of $1$ if and only if it is a directed series-parallel graph. We also study the computational complexity of finding a directed minor and computing the serial-parallel width.

==> network_minor_not_embed.tex <==
%\documentclass[]{article}
%\usepackage{tikz}
%\usepackage{pgfplots}
%%\usepackage{tikz}%,fullpage}
%\usetikzlibrary{arrows,%
                %petri,%
                %topaths}%
%\usepackage{tkz-berge}
%\usepackage[position=top]{subfig}
%\def\GG{\mathbb{G}}
%\input{defs}
%\begin{document}
\begin{figure}
\centering


%where
%\captionsetup[subfigure]{labelformat=empty}
%\subfloat[$c(x)$]{ 
\begin{tikzpicture}[scale=0.75,transform shape]
  \Vertex[x=3.5,y=3]{s}
  \Vertex[x=0.5,y=2.7]{a}
  \Vertex[x=2,y=1.8]{b}
  \Vertex[x=2,y=0]{t}
  \tikzstyle{VertexStyle}=[fill=black!20!white]
  
  \tikzstyle{LabelStyle}=[fill=white,sloped]
  \tikzstyle{EdgeStyle}=[->]
  \Edge(s)(a)
  \Edge(s)(b)
  \Edge(s)(t)
	\Edge(a)(b)
	\Edge(a)(t)
	\Edge(b)(t)
  \end{tikzpicture}
%}
\quad\quad
\begin{tikzpicture}[scale=0.75,transform shape]
 \Vertex[x=3.5,y=3]{s}
  \Vertex[x=0.5,y=2.7]{a}
  \Vertex[x=2,y=1.8]{b}
  \Vertex[x=2,y=0.8]{x}
	\Vertex[x=2,y=-.4]{y}
  \tikzstyle{VertexStyle}=[fill=black!20!white]
  
  \tikzstyle{LabelStyle}=[fill=white,sloped]
  \tikzstyle{EdgeStyle}=[->]
  \Edge(s)(a)
  \Edge(s)(b)
  \Edge(s)(x)
	\Edge(a)(b)
	\Edge(a)(y)
	\Edge(b)(x)
	\Edge(x)(y)
  \end{tikzpicture}



\caption{\label{fig:embed_minor}The graph $G'$ (left) and $G$ (right). Note that in $G'$ there is a node with indegree~3, and a node with indegree at least 3 will continue to exist after any embedding operation (split edge, add edge, extend terminal). Thus $G'$ cannot be d-embedded in $G$, where all nodes have indegree at most 2. In contrast, we can obtain $G'$ from $G$ by contracting the edge $(x,y)$. Thus $G'$ is a d-minor of $G$.}
\end{figure}
%\end{document}

